PILLAR: an AI-Powered Privacy Threat Modeling Tool

The rapid evolution of Large Language Models (LLMs) has unlocked new possibilities for applying artificial intelligence across a wide range of fields, including privacy engineering. As modern applications increasingly handle sensitive user data, safeguarding privacy has become more critical than ever. To protect privacy effectively, potential threats need to be identified and addressed early in the system development process. Frameworks like LINDDUN offer structured approaches for uncovering these risks, but despite their value, they often demand substantial manual effort, expert input, and detailed system knowledge. This makes the process time-consuming and prone to errors. Current privacy threat modeling methods, such as LINDDUN, typically rely on creating and analyzing complex data flow diagrams (DFDs) and system descriptions to pinpoint potential privacy issues. While these approaches are thorough, they can be cumbersome, relying heavily on the precision of the data provided by users. Moreover, they often generate a long list of threats without clear guidance on how to prioritize them, leaving developers unsure of where to focus their efforts. In response to these challenges, we introduce PILLAR (Privacy risk Identification with LINDDUN and LLM Analysis Report), a new tool that integrates LLMs with the LINDDUN framework to streamline and enhance privacy threat modeling. PILLAR automates key parts of the LINDDUN process, such as generating DFDs, classifying threats, and prioritizing risks. By leveraging the capabilities of LLMs, PILLAR can take natural language descriptions of systems and transform them into comprehensive threat models with minimal input from users, reducing the workload on developers and privacy experts while improving the efficiency and accuracy of the process.

==> Sections/5-Related_work.tex <==
\section{Related Work}
\label{sec:related}

The integration of LLMs into the field of cybersecurity has garnered considerable attention due to their ability to process and analyze vast datasets. As cyber threats become more sophisticated, the cybersecurity domain increasingly turns to these advanced models to strengthen defenses. Cybersecurity professionals continually seek innovative solutions to implement robust policies and enhance technological safeguards~\cite{kaur}. These efforts are essential for preventing the unauthorized disclosure of sensitive information, unauthorized access, and various forms of data manipulation~\cite{yang}. 

The ability of LLMs to adapt and scale is particularly valuable for addressing the growing complexity of cyber threats. The following sections highlight key applications of LLMs in cybersecurity, summarize findings from recent research, and discuss notable tools leveraging LLMs to improve security. Applications of LLMs in cybersecurity include:

\begin{itemize}
    \item \textbf{Vulnerability Detection:} LLMs can analyze code and security advisories to identify potential vulnerabilities in software systems.
    \item \textbf{Malware Analysis:} These models assist in classifying and analyzing malware by recognizing complex data patterns.
    \item \textbf{Network Intrusion Detection:} LLMs can process network traffic data to detect anomalies that may signal potential intrusions.
    \item \textbf{Phishing Detection:} By analyzing textual patterns, LLMs can detect phishing attempts with greater precision than traditional methods~\cite{xu2024large, motlagh}.
\end{itemize}

Although the application of LLMs shows promising advancements, research suggests challenges remain, such as the need for larger training datasets and more interpretable models. Future work is expected to focus on improving model explainability, addressing privacy concerns, and developing proactive defense mechanisms against cyber threats.

One significant application of LLMs in network security is web fuzzing. For example, Liang et al.~\cite{liang2023generative} proposed GPTFuzzer, which uses an encoder-decoder architecture to generate effective payloads for web application firewalls (WAFs). It specifically targets vulnerabilities such as SQL injection, cross-site scripting (XSS), and remote code execution (RCE) by generating fuzz test cases. Another notable use of LLMs is in detecting network traffic anomalies. Liu et al.~\cite{liu2023malicious} developed a method to detect malicious URLs by leveraging LLMs to extract hierarchical features. This work extends the use of LLMs in intrusion detection tasks to the user level, demonstrating their generality and effectiveness in intrusion and anomaly detection.

As cyber threats grow in complexity, traditional Cyber Threat Intelligence (CTI) methods struggle to keep pace. AI-based solutions, including LLMs, offer an opportunity to automate and enhance several tasks, ranging from data ingestion to resilience verification. LLMs have shown promise in generating CTI from various sources, including network security texts (e.g., books, blogs, news)~\cite{aghaei2022securebert}, generating structured reports from unstructured data~\cite{siracusano2023time}, and extracting intelligence from network security entity graphs~\cite{perrina2023agir}. Aghaei et al.~\cite{aghaei2023automated} introduced CVEDrill, which generates priority recommendation reports for cybersecurity threats and predicts their potential impact. Furthermore, Moskal et al.~\cite{moskal2023llms} examined the use of ChatGPT in assisting or automating decision-making in response to threat behaviors, illustrating the potential of LLMs in handling simple network attack scenarios.

In the context of vulnerability detection, Liu et al.~\cite{liu2023harnessing} proposed LATTE, which combines LLMs with automated binary taint analysis. LATTE overcomes the limitations of traditional taint analysis, which often requires manual customization of taint propagation and vulnerability inspection rules. Phishing and scam detection is another area where LLMs demonstrate significant utility. Labonne et al.~\cite{labonne2023spam} highlighted the effectiveness of LLMs in spam email detection, showcasing their superiority over traditional machine learning approaches. Additionally, Cambiaso et al.~\cite{cambiaso2023scamming} presented an innovative study suggesting that LLMs can mimic human interactions with scammers in an automated yet meaningless manner, wasting scammers’ time and resources, and thereby reducing the impact of scam emails.

Detection and Intelligence Analysis for New Alerts\footnote{\url{https://github.com/dwillowtree/diana}} (DIANA) is another recently developed tool that automates the creation of detections from threat intelligence using LLMs. In the context of modeling security threats, STRIDE-GPT\footnote{\url{https://github.com/mrwadams/stride-gpt}} is another advanced tool that generates threat models and attack trees for a given application based on the STRIDE methodology. AttackGen\footnote{\url{https://github.com/mrwadams/attackgen}} is a cybersecurity incident response testing tool that leverages the power of large language models and the comprehensive MITRE ATT\&CK framework\footnote{\url{https://attack.mitre.org/}}. The tool generates tailored incident response scenarios based on user-selected threat actor groups and your organisation's details.  

A framework that leverages multiple intelligent LLM agents working collaboratively can enhance the efficiency and effectiveness of handling complex tasks. This approach addresses various challenges such as security risks, scalability, and system evaluation, showcasing the potential for advanced applications in cybersecurity~\cite{talebirad2023multi}. For instance, authors in~\cite{song2024audit} introduced Audit-LLM, a multi-agent log-based insider threat detection (ITD) framework comprising three collaborative agents, where it detects malicious user activities by auditing log entries.


